Requirements Engineering for a Web-based Research, Technology & Innovation Monitoring Tool

With the increasing significance of Research, Technology, and Innovation (RTI) policies in recent years, the demand for detailed information about the performance of these sectors has surged. Many of the current tools are limited in their application purpose. To address these issues, we introduce a requirements engineering process to identify stakeholders and elicitate requirements to derive a system architecture, for a web-based interactive and open-access RTI system monitoring tool. Based on several core modules, we introduce a multi-tier software architecture of how such a tool is generally implemented from the perspective of software engineers. A cornerstone of this architecture is the user-facing dashboard module. We describe in detail the requirements for this module and additionally illustrate these requirements with the real example of the Austrian RTI Monitor.

==> fmt.tex <==
\usepackage{fancyhdr}
\usepackage{amsthm}%
\usepackage{mathrsfs}%
\usepackage[title]{appendix}%
\usepackage{manyfoot}%
\usepackage{algorithm}%
\usepackage{algorithmicx}%
\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage{amsmath,amssymb,amsfonts} %%assymb breaks the acm template
\usepackage{url}
\usepackage[inline]{enumitem}

\usepackage{booktabs} % For formal tables                  
%\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{hyperref}
\usepackage{balance}
\usepackage{tabularx}
\usepackage[acronym]{glossaries}

\usepackage{booktabs}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{caption}
%\usepackage{subfigure}
\usepackage{subcaption}
\usepackage[export]{adjustbox}
\usepackage{tabularx}
\usepackage{tikz}
\usepackage{float}
%\usepackage[shortlabels]{enumitem}
\usepackage[font=small]{caption}

\usepackage{csquotes}
\MakeOuterQuote{"}




\usepackage{xcolor}
\usepackage{url}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{array}
\usepackage{color}
\usepackage{wasysym}
\usepackage{verbatim}
\usepackage{bigstrut}
\usepackage{multirow}
%\usepackage{amsmath}
\usepackage{setspace}
\usepackage{tabularx}
\usepackage{url}
\usepackage{xspace}
\usepackage{pifont}
\usepackage{subcaption}
\usepackage[font=footnotesize]{caption}%,labelfont=bf]{caption}
\usepackage{array,booktabs}
\usepackage{soul}
\usepackage{vcell}
\usepackage{pifont}
\usepackage{afterpage}
\usepackage{rotating}
\usepackage{wrapfig}
\usepackage{caption}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{enumitem}
\usepackage{lipsum}
%\usepackage{xcolor}
\usepackage{balance}
\usepackage{tikz}
\usepackage{hyperref}














\definecolor{commentGreen}{RGB}{128,127,41}
\definecolor{stringGreen}{RGB}{0,127,38}
\definecolor{keywordRed}{RGB}{151,0,11}
\definecolor{typePurple}{RGB}{128,3,82}
\definecolor{variableBlue}{RGB}{0,0,255}
\definecolor{annotationRed}{RGB}{198,4,38}
\definecolor{annotationBlue}{RGB}{32,21,223}

\newcommand{\etal}{\emph{et~al.}\xspace}

\newcommand{\citesec}[1]{Section~\ref{sec:#1}}
\newcommand{\citefig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\citealgo}[1]{\textsc{Listing}~\ref{algo:#1}}
\newcommand{\citelisting}[1]{\textsc{Listing}~\ref{lst:#1}}
\newcommand{\citetable}[1]{{Table}~\ref{tab:#1}}
\newcommand{\citedef}[1]{\textsc{Definition}~\ref{def:#1}}
\newcommand{\citesecs}[2]{Sections~\ref{sec:#1} and~\ref{sec:#2}}

% \newcommand{\mv}[1]{{\textcolor{orange}{#1}}}%orange
% \newcommand{\ig}[1]{{\textcolor{blue}{#1}}}%blue
% \newcommand{\ta}[1]{{\textcolor{green}{#1}}}%green

% \newcommand{\fwname}{{\textcolor{purple} EduComp}\xspace}%orange


\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash}p{#1}} 
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash}p{#1}} 


\newcommand{\bullitem}[1]{\noindent$\bullet$\textbf{ #1}}

\newcommand{\intqte}[1]{\emph{#1}}


\newcommand{\archname}{{SoS-PuDZ}\xspace}
\newcommand{\pubtop}[1]{{\texttt{\small #1}\xspace}}



\newcommand{\MtoH}{\textbf{$[M \rightarrow H]$}\xspace}
\newcommand{\HtoM}{\textbf{$[H \rightarrow M]$}\xspace}

\newcommand{\jch}[1]{{\textcolor{blue}{#1}}} %blue
\newcommand{\ankit}[1]{{\textcolor{purple}{#1}}} %purple
\newcommand{\mv}[1]{{\textcolor{orange}{#1}}}%orange
\newcommand{\mkhmt}{{\it MAPE-K$_{HMT}$}\xspace}
\newcommand{\DR}{{\it Drone Response}\xspace}
\newcommand{\DRx}{{\it Drone Response}}
\newcommand{\pudz}{{\it PuDZ}\xspace}


\newcommand{\ttformat}[1]{{\texttt{\small #1}}}

\definecolor{alizarin}{rgb}{0.82, 0.1, 0.26}
\newcommand{\hlt}[1]{{\textcolor{alizarin}{#1}}}%orange
\newcommand{\markphase}{ \CIRCLE}
\hyphenation{autono-mous}


